An Open source Implementation of ITU-T Recommendation P.808 with Validation

The ITU-T Recommendation P.808 provides a crowdsourcing approach for conducting a subjective assessment of speech quality using the Absolute Category Rating (ACR) method. We provide an open-source implementation of the ITU-T Rec. P.808 that runs on the Amazon Mechanical Turk platform. We extended our implementation to include Degradation Category Ratings (DCR) and Comparison Category Ratings (CCR) test methods. We also significantly speed up the test process by integrating the participant qualification step into the main rating task compared to a two-stage qualification and rating solution. We provide program scripts for creating and executing the subjective test, and data cleansing and analyzing the answers to avoid operational errors. To validate the implementation, we compare the Mean Opinion Scores (MOS) collected through our implementation with MOS values from a standard laboratory experiment conducted based on the ITU-T Rec. P.800. We also evaluate the reproducibility of the result of the subjective speech quality assessment through crowdsourcing using our implementation. Finally, we quantify the impact of parts of the system designed to improve the reliability: environmental tests, gold and trapping questions, rating patterns, and a headset usage test.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> tab_others.tex <==
The Pearson cross correlation matrix is shown in Table X.
\begin{center}
    \begin{tabular}{| c| c | c | c | c | c |}
    % Babak: I think this table does not add further information and can be removed.
    \hline
        &    Run1&	Run2&	Run3&	Run4&	Run5    \\ \hline
    Run1&	1.000&	&       &       &   			\\ \hline
    Run2&	0.995&	1.000&  &       &               \\ \hline
    Run3&	0.998&	0.994&	1.000&  &	            \\ \hline
    Run4&	0.995&	0.990&	0.992&	1.000&	        \\ \hline
    Run5&	0.995&	0.998&	0.997&	0.993&	1.000   \\ \hline \hline
    Average & 0.995 \\ 
    \hline
    \end{tabular}
\end{center}

The rank for each run is shown in Table X.
\babak{Is it necessary to report ranks? one can read it from the first table.}
% include CI in SRCC? Also see paper from Babak

\begin{center}
    % Babak: I think this table does not add further information and can be removed.
    \begin{tabular}{| c| c | c | c | c | c |}
    \hline
    Name&	Run1&	Run2&	Run3&	Run4&	Run5    \\ \hline
    Model1&	1&	1&	1&	1&	1                   \\ \hline
    Model2&	3&	2&	3&	3&	2                   \\ \hline
    Model3&	2&	3&	2&	2&	3                   \\ \hline
    Model4&	4&	4&	4&	4&	4                   \\ \hline
    Noisy&	5&	5&	5&	5&	5                   \\ \hline
    \end{tabular}
\end{center}

The SRCC matrix is shown in Table X.

\begin{center}
    \begin{tabular}{| c| c | c | c | c | c |}
    % Babak: I think this table does not add further information and can be removed.
    \hline
	&       Run1&   Run2&	Run3&	Run4&	Run5    \\ \hline
    Run1&	1.00&      &       &       &			    \\ \hline
    Run2&	0.90&    1.00&      &       &             \\ \hline			
    Run3&	1.00&	0.90&	1.00&      &             \\ \hline		
    Run4&	1.00&	0.90&	1.00&	  1.00&          \\ \hline	
    Run5&	0.90&	1.00&    0.90&      0.90&	1.0     \\ \hline \hline
    Average	& 0.940 \\ \hline				
    \end{tabular}
\end{center}
